Elly: A Real-Time Failure Recovery and Data Collection System for Robotic Manipulation

Even the most robust autonomous behaviors can fail. The goal of this research is to both recover and collect data from failures, during autonomous task execution, so they can be prevented in the future. We propose haptic intervention for real-time failure recovery and data collection. Elly is a system that allows for seamless transitions between autonomous robot behaviors and human intervention while collecting sensory information from the human's recovery strategy. The system and our design choices were experimentally validated on a single arm task -- installing a lightbulb in a socket -- and a bimanual task -- screwing a cap on a bottle -- using two 7-DOF manipulators equipped 4-finger grippers. In these examples, Elly achieved over 80% task completion during a total of 40 runs.

==> list.tex <==
Summary of references by topic: 
\begin{itemize}

    \item Model based primitives: 
    
    \item , learning for controls \cite{Coates2008LearningDemonstrations}, learning to generalize for tenis \cite{Mulling2013LearningTennis}, learning with task-parametrized generative models \cite{}
    
    \item HRC: probabilistic primitives \cite{}, 
    
    \item Generalizing: scalable deep RL \cite{KalashnikovScalableManipulation}
    
    \item Learning:imitation for humanoids \cite{Ijspeert2002MovementRobots}, learning dynamics (of doors) \cite{Endres2013LearningManipulation}, learning what and where (looks super cool) \cite{ShridharCLIPORT:Manipulation}
    
    \item haptics: haptic switching , margot device , 
    
    \item manipulation: hanging stuff \cite{You2021OmniHang:Estimation}, 
    
    \item planning: predicates toki \cite{Migimatsu2021GroundingActions}
    
    \item object-centric:   
    
    \item grasping:
    
    \item primitives: task-specific \cite{Ude2010Task-specificPrimitives}, manipulation primitives for composing skills '97 \cite{Morrow1997ManipulationSkills}, '90 \cite{Curtis1990PrimitivesControl}, compliant movement primitives review \cite{Denisa2016APrimitives}, learning motion primitive goals \cite{Stulp2011LearningManipulation}, RL with sequences of primitives \cite{Stulp12RLprimitiveSequences}, probabilistic primitives \cite{Gomez-Gonzalez2017AdaptationPrimitives}, modular RL kunal \cite{Andreas2017ModularSketches}, Ellen \cite{Khansari2016AdaptiveUncertainty}, learning to sequence from demo \cite{Manschitz2014LearningDemonstrations}, probabilistic movement primitives \cite{Paraschos2018UsingRobotics}
    
    
    \item stochastic control: \cite{Theodorou2011IterativeControl}
    
    \item contact: state estimation in contact \cite{Wirnshofer2019StateManipulation}, paper with Mika \cite{Jorda2019Contact-DrivenOperation}
    
    \item Oussama: 
    
\end{itemize}
